Fairness-Aware Neural R\'eyni Minimization for Continuous Features

The past few years have seen a dramatic rise of academic and societal interest in fair machine learning. While plenty of fair algorithms have been proposed recently to tackle this challenge for discrete variables, only a few ideas exist for continuous ones. The objective in this paper is to ensure some independence level between the outputs of regression models and any given continuous sensitive variables. For this purpose, we use the Hirschfeld-Gebelein-R\'enyi (HGR) maximal correlation coefficient as a fairness metric. We propose two approaches to minimize the HGR coefficient. First, by reducing an upper bound of the HGR with a neural network estimation of the $\chi^{2}$ divergence. Second, by minimizing the HGR directly with an adversarial neural network architecture. The idea is to predict the output Y while minimizing the ability of an adversarial neural network to find the estimated transformations which are required to predict the HGR coefficient. We empirically assess and compare our approaches and demonstrate significant improvements on previously presented work in the field.

==> trash.tex <==
\section{Dual Representation of $\chi^2$}

\begin{theorem}
The $\chi^2$ divergence admits the following representation: 
\begin{eqnarray}
\chi^2(P,Q) = \sup_{f: \Omega \rightarrow \mathbb{R}} E_{P}(f) - T(f,Q) 
\end{eqnarray}
with  
\begin{eqnarray}
T(f,Q) =  E_{Q}(f)+\frac{1}{4}E_{Q}(f^2)
\end{eqnarray}
where the supremum is taken over all functions $f$ such that the expectations are finite.
\end{theorem}
\begin{proof}
Equipped with the $\tau_F$ -topology, $M_\mathcal{F}$ is a Hausdorff locally convex topological vector spaces. Its topological dual space is the set of all mappings $P \mapsto \int f dP$ when $f$ belongs to $\langle F \in B_{b} \rangle$.

The function $P \in [M_\mathcal{F}; \tau_\mathcal{F}] \mapsto \chi^2(P, Q)$ is lower semi-continuous (l.s.c.); see , Proposition 2.2. This allows to use the Legendre Fenchel theory in order to represent the mapping $P \mapsto \chi^2(P, Q)$ as the upper envelope of its support hyperplanes.
On $\langle F \in B_{b} \rangle$ define the Fenchel–Legendre transform of $\chi^2(·, Q )$

$T(f,Q) := sup_{P \in M_{f}} \int f dP - \chi^2(P, Q)$
\end{proof}




%Comme attendu figure \ref{fig:superficie}, la tendance de la prédiction du coût moyen est strictement croissante par rapport à la superficie (courbe bleu).




\begin{table*}[h]
\caption{Data sets used for the experiments}
\label{tab:description_of_data_sets}
\centering
\begin{tabular}{lllll}
\hline
\multicolumn{1}{c}{Data set} & \multicolumn{1}{c}{\# Observations} & \multicolumn{1}{c}{\# Features} & \multicolumn{1}{c}{Target} & \multicolumn{1}{c}{Sensitive}  \\ \hline
US Census                      &                 74,000                &         37        &                    Children under poverty level per population               &                  Gender                                    \\
         \\ \hline
         Motor Insurance                       &                    36,311                 &                   15              &                    Average claim cost                      &                  Age                                     \\
                            \\ \hline

         Crime                      &                   1,994                &         128        &                    Violent crimes per population               &                  Race                                    \\
         \\ \hline
Medical Cost                       &                    1,338                 &                   7              &                    Health care cost         &                  BMI                                   \\
                             \\ \hline


\end{tabular}
\\[5pt] 
Description of the data sets: number of observations, number of features, target, sensitive attribute.
\end{table*}

\begin{table*}[!h]
\caption{Results for Demographic Parity}
\label{tab:results_demographic_parity}
\centering



\begin{tabular}{|l|l|l|l|l|l|l|l|l|}

\cline{1-9} 
                                
& & MSE & HGR\_NN & HGR\_KDE & HGR\_RDC & $\chi^2$\ KDE & $\chi^2$\ NN & MSE QUANTILE \\ 
\hline
\multirow{5}{*}{\rotatebox[origin=c]{90}{US Census}}
& Standard NN & 0.274  & 0.212 & 0.181 & 0.217 & 0.036  & 0.032 &  0.0591507 (0.0048071) \\
%\cline{2-9} 
& Fair HGR & \textbf{0.482}  & \textbf{0.057} & \textbf{0.047} & \textbf{0.044} & \textbf{0.005} &   \textbf{0.003} & \textbf{0.011 (0.0002610)} \\
%\cline{2-9} 
& Fair $\chi^2$ & 0.535  & 0.069 & 0.048 & 0.044  &    0.004 & 0.002 & 0.00786 (8.38838) \\
%\cline{2-9} 
& Mary2019~\cite{mary2019fairness} & 0.541  & 0.075 & 0.0613 & 0.078 & 0.005 & 0.003 & 0.0191416 (0.0007781) \\ 
%\cline{2-9} 
& MINE~\cite{belghazi2018mutual} & 0.537 & 0.058 & 0.048 & 0.045 & 0.005 & 0.003 & 0.012 (0.0002713) \\
%\cline{2-9} 
& Fair Pearson &   0.544   & 0.202  & 0.151 & 0.211   & 0.013  & 0.010 &  0.1141 (0.03113) \\ 

\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{Motor}}
& Standard NN & 0.945   & 0.201 & 0.175 & 0.200 & 0.035 & 0.029 & 0.0075 (0.00010)\\ 
%\cline{2-9} 
& Fair HGR & 0.971   & 0.072 & 0.058 &  0.066 & 0.006 & 0.004 & 0.001915 (1.428661) \\ 
%\cline{2-9}
& Fair $\chi^2$ & \textbf{0.975}  & \textbf{0.076} & \textbf{0.067} & \textbf{0.067} & \textbf{0.008} & \textbf{0.005} & 0.0037 (1.90383979) \\ 
%\cline{2-9}
& Mary2019~\cite{mary2019fairness} & 0.979   & 0.077 & 0.059 & 0.067 & 0.006 & 0.005 & 0.0037 (2.36651) \\ 
%\cline{2-9}
& MINE~\cite{belghazi2018mutual} & 0.982 & 0.078 & 0.068 & 0.069 & 0.008 & 0.006 & 0.0042 (2.024752)\\
& Fair Pearson &      &   &   &  &  &  &  \\ 

\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{Crime}}
& Standard NN                        &    0.384     &  0.732 &  0.525 &  0.731 & 0.319  &    0.352 &  0.35311 (0.154919) \\ %\cline{2-9}
& Fair HGR    &     0.781     &  0.356 &  0.097  &  0.171  &  0.014   & 0.064 & 0.03907 (0.002807)          \\ 
%\cline{2-9}
& Fair $\chi^2$  &   0.769     &  0.396 &  0.112  &  0.193  &  0.021   & 0.082 & 0.14732 (0.010023)   \\ 
%\cline{2-9}
& Mary2019~\cite{mary2019fairness}    &   0.778  &   0.371    &  0.115 &  0.177  &  0.022   &   0.09 &      0.06369 (0.00661)    \\ 
%\cline{2-9}
& MINE~\cite{belghazi2018mutual}  &   0.782     &  0.395 &  0.110  &  0.201 &  0.022   & 0.079 & 0.13632 (0.009542)  \\ 


\hline
\end{tabular}
\centering
\\
Comparing our approach with different common fair algorithms by accuracy (MSE) and fairness (HGR\_NN, HGR\_KDE, HGR\_RDC, $\chi^2$\ KDE, $\chi^2$\ NN, MI)
for the US Census, Motor Insurance and Crime data set.
\end{table*}





\begin{table*}[!h]
\caption{Results for Equalized Residuals}
\label{tab:results_equalized_odds}
\centering



\begin{tabular}{|l|l|l|l|l|l|l|l|l|}

\cline{1-9} 
& & MSE & HGR\_NN & HGR\_KDE & HGR\_RDC & $\chi^2$\ KDE & $\chi^2$\ NN & MSE\_Quantile \\ 
\hline
\multirow{6}{*}{\rotatebox[origin=c]{90}{US Census}}
& Standard NN    &   0.274   &  0.157  &  0.098  &  0.122   & 0.012   &  0.010  & 0.00797(0.00015)  \\
%\cline{2-9} 
& Fair HGR NN   &  0.334 & \textbf{0.068}   &  0.053  & 0.055 & \textbf{0.004}  &  0.003   &  0.0033 (1.94897 10-5) \\
%\cline{2-9} 
& Fair $\chi^2$ NN     &  \textbf{0.384}    &  0.084  &  \textbf{0.054}  & \textbf{0.057} & \textbf{0.005}  &  \textbf{0.003} &   0.005946 (6.4135722 10-5)
\\
%\cline{2-9} 
& Mary2019~\cite{mary2019fairness}     &  0.408  &  0.092  & 0.049  & 0.063  & 0.005 & 0.003   &    0.00861 (0.000139) \\ 
%\cline{2-9} 
& Fair MINE NN~\cite{belghazi2018mutual}     &  0.406    &  0.083  &  0.055 & 0.057 & 0.005  &  0.003 &  0.007632 (0.0001111)  \\ 
%\cline{2-9} 
& Fair Pearson &   0.421   & 0.325  & 0.249  & 0.305 &  0.092 &  0.078   &  0.172 (0.04604) \\ 

\hline

\multirow{6}{*}{\rotatebox[origin=c]{90}{Motor}}
& Standard NN     &  0.945     &  0.145 &  0.102  & 0.123 & 0.013  &  0.010 &   0.07531 (0.01036) \\ 
%\cline{2-9} 
& Fair HGR NN    &   0.991  & \textbf{0.102}  &  0.082   & 0.092 & 0.010  &   0.008  &  0.0107 (0.00041) \\ 
%\cline{2-9}
& Fair $\chi^2$ NN   &    1.011  & 0114   &   0.081 & \textbf{0.077} &  \textbf{0.010}  &  0.008 &   0.0138(0.00053)  \\ 
%\cline{2-9}
& Mary2019~\cite{mary2019fairness}     &   1.019    &   0.111 &  0.079  & 0.098  &  0.009   &    0.006  & 0.01482 (0.00056) \\ 
%\cline{2-9}
& Fair MINE NN ~\cite{belghazi2018mutual}     &    1.024  & 0121   &   0.091 & \textbf{0.092} &  \textbf{0.012}  &  0.012 &  0.03116 (0.00091)    \\
%\cline{2-9}
& Fair Pearson    &     &   &    &  &   &   &  \\
\hline

\multirow{5}{*}{\rotatebox[origin=c]{90}{Crime}}
& Standard NN      &   0.385  &  0.472   &  0.244    & 0.440 & 0.092  &  0.096 & 0.0465 (0.0029)  \\ %\cline{2-9}
& Fair HGR NN  &   0.583    & 0.382   &    0.1514 & 0.222 & 0.038  & 0.092   & 0.02812 (0.0027)  \\ 
%\cline{2-9}
& Fair $\chi^2$ NN  &   0.574    & 0.333   &    0.1317 & 0.201 & 0.034  & 0.088   & 0.03232 (0.0034)   \\ 
%\cline{2-9}
& Mary2019~\cite{mary2019fairness}     &   0.579    & 0.382   &    0.1514 & 0.222 & 0.038  & 0.092   & 0.05837 (0.00492)   \\ 
%\cline{2-9}
& Fair MINE NN~\cite{belghazi2018mutual}  &   0.583    & 0.413  &    0.161 & 0.232 & 0.041  & 0.098  & 0.0 \\ 


\hline
\end{tabular}
\centering
\\
Comparing our approach with different common fair algorithms by accuracy (MSE) and fairness (HGR\_NN, HGR\_KDE, HGR\_RDC, $\chi^2$\ KDE, $\chi^2$\ NN, MI) for the US Census, Motor Insurance and Crime data set.
\end{table*}



\begin{figure}[h]
  \centering
  \subfloat[Sine function]{
  \includegraphics[frame,width=0.24\textwidth]{pictures/HGR_NN_sinus.pdf}
  %\hspace{0.01cm}
  %\includegraphics[frame,width=0.23\textwidth]{pictures/HGR2_sine2.pdf}
  \label{empirical_1}
  %\includegraphics[frame,width=0.33\textwidth]{pictures/HGR2_sine_tanh.pdf}
  %\hspace{0.01cm}
  %\includegraphics[frame,width=0.33\textwidth]{pictures/HGR2_sine2_tanh.pdf}
  %\label{empirical_2}
  }
  \subfloat[Square function]{
  \includegraphics[frame,width=0.24\textwidth]{pictures/HGR_NN_X2.pdf}
  %\hspace{0.01cm}
  %\includegraphics[frame,width=0.23\textwidth]{pictures/HGR_X2_2.pdf}
  \label{empirical_3}
  }  \\
  \hspace{0.07cm}
  \subfloat[Normal function]{
  \includegraphics[frame,width=0.24\textwidth]{pictures/HGR_NN_normal.pdf}
  %\hspace{0.01cm}
  %\includegraphics[frame,width=0.23\textwidth]{pictures/HGR2_normal2.pdf}
  \label{empirical_4}
  }
 \subfloat[$sin(0.2^X)$]{
  \includegraphics[frame,width=0.24\textwidth]{pictures/HGR_NN_funcg.pdf}
  %\hspace{0.01cm}
  %\includegraphics[frame,width=0.23\textwidth]{pictures/HGR2_normal2.pdf}
  \label{empirical_4}
  }
  \caption{Empirical assessments}
  \label{fig:empirical_assessments}

\end{figure}
